Efficient model compression with Random Operation Access Specific Tile (ROAST) hashing

Advancements in deep learning are often associated with increasing model sizes. The model size dramatically affects the deployment cost and latency of deep models. For instance, models like BERT cannot be deployed on edge devices and mobiles due to their sheer size. As a result, most advances in Deep Learning are yet to reach the edge. Model compression has sought much-deserved attention in literature across natural language processing, vision, and recommendation domains. This paper proposes a model-agnostic, cache-friendly model compression approach: Random Operation Access Specific Tile (ROAST) hashing. ROAST collapses the parameters by clubbing them through a lightweight mapping. Notably, while clubbing these parameters, ROAST utilizes cache hierarchies by aligning the memory access pattern with the parameter access pattern. ROAST is up to $\sim 25 \times$ faster to train and $\sim 50 \times$ faster to infer than the popular parameter sharing method HashedNet. Additionally, ROAST introduces global weight sharing, which is empirically and theoretically superior to local weight sharing in HashedNet, and can be of independent interest in itself. With ROAST, we present the first compressed BERT, which is $100\times - 1000\times$ smaller but does not result in quality degradation. These compression levels on universal architecture like transformers are promising for the future of SOTA model deployment on resource-constrained devices like mobile and edge devices

==> tables/ext_t1.tex <==
\begin{table}[]
\begin{tabular}{|c|c|ccc|cll|cll|cll|cll|cll|}
\hline
\textbf{d}           & \textbf{Architecture}     & \multicolumn{3}{c|}{\textbf{Original}}                          & \multicolumn{3}{l|}{\textbf{RzLinear-2x}}                                          & \multicolumn{3}{c|}{\textbf{RzLinear-4x}}                                          & \multicolumn{3}{c|}{\textbf{RzLinear-8x}}                                          & \multicolumn{3}{c|}{\textbf{RzLinear-12x}}                                         & \multicolumn{3}{c|}{\textbf{RzLinear-16x}}                                         \\ \hline
                     &                           & \multicolumn{1}{c|}{P@1}   & \multicolumn{1}{c|}{P@3}   & P@5   & \multicolumn{1}{c|}{P@1}   & \multicolumn{1}{c|}{P@3}   & \multicolumn{1}{c|}{P@5} & \multicolumn{1}{c|}{P@1}   & \multicolumn{1}{c|}{P@3}   & \multicolumn{1}{c|}{P@5} & \multicolumn{1}{c|}{P@1}   & \multicolumn{1}{c|}{P@3}   & \multicolumn{1}{c|}{P@5} & \multicolumn{1}{c|}{P@1}   & \multicolumn{1}{c|}{P@3}   & \multicolumn{1}{c|}{P@5} & \multicolumn{1}{c|}{P@1}   & \multicolumn{1}{c|}{P@3}   & \multicolumn{1}{c|}{P@5} \\ \hline
LF-AmazonTitles-131K & 40K-500-131K              & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}      &       & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          \\ \hline
LF-AmazonTitles-131K & 40K-500-500-500-131K      & \multicolumn{1}{c|}{0.210} & \multicolumn{1}{c|}{0.139} & 0.097 & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{0.219} & \multicolumn{1}{l|}{0.147} & 0.104                    & \multicolumn{1}{c|}{0.202} & \multicolumn{1}{l|}{0.135} & 0.096                    & \multicolumn{1}{c|}{0.188} & \multicolumn{1}{l|}{0.125} & 0.090                    & \multicolumn{1}{c|}{0.174} & \multicolumn{1}{l|}{0.115} & 0.082                    \\ \hline
Eurlex-4K            & 5000-500-3993             & \multicolumn{1}{c|}{0.766} & \multicolumn{1}{c|}{0.624} & 0.517 & \multicolumn{1}{c|}{0.759} & \multicolumn{1}{l|}{0.617} & 0.505                    & \multicolumn{1}{c|}{0.739} & \multicolumn{1}{l|}{0.593} & 0.484                    & \multicolumn{1}{c|}{0.724} & \multicolumn{1}{l|}{0.567} & 0.460                    & \multicolumn{1}{c|}{0.689} & \multicolumn{1}{l|}{0.540} & 0.440                    & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          \\ \hline
Eurlex-4K            & 5000-500-500-500-500-3993 & \multicolumn{1}{c|}{0.692} & \multicolumn{1}{c|}{0.544} & 0.440 & \multicolumn{1}{c|}{0.663} & \multicolumn{1}{l|}{0.52}  & 0.424                    & \multicolumn{1}{c|}{0.674} & \multicolumn{1}{l|}{0.525} & 0.429                    & \multicolumn{1}{c|}{0.653} & \multicolumn{1}{l|}{0.509} & 0.412                    & \multicolumn{1}{c|}{0.665} & \multicolumn{1}{l|}{0.513} & 0.418                    & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          \\ \hline
Delicious-200K       & 782K-500-500-500-500-200K & \multicolumn{1}{c|}{0.387} & \multicolumn{1}{c|}{0.365} & 0.352 & \multicolumn{1}{c|}{0.384} & \multicolumn{1}{l|}{0.356} & 0.350                    & \multicolumn{1}{c|}{0.384} & \multicolumn{1}{l|}{0.365} & 0.352                    & \multicolumn{1}{c|}{0.385} & \multicolumn{1}{l|}{0.364} & 0.354                    & \multicolumn{1}{c|}{0.386} & \multicolumn{1}{l|}{0.366} & 0.353                    & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          \\ \hline
                     &                           & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}      &       & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          \\ \hline
                     &                           & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}      &       & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          \\ \hline
                     &                           & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}      &       & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          & \multicolumn{1}{c|}{}      & \multicolumn{1}{l|}{}      &                          \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}

==> tables/kernel_times.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\caption{Inference time and training time of ROAST-MM kernels compared to Full matrix multiplication and HashedNet.
\roach-MM kernel is much faster than HashedNet kernel due to coalesced memory accesses. For large matrices, \roach-MM can be up to {\color{red}60$\times$} faster than HashedNet kernel.}
\label{tab:kerneltimes}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|r|rrrrrrr|rrrrrrr|}
\hline
                                                & \multicolumn{1}{l|}{}                                                         & \multicolumn{7}{c|}{\textbf{Inference (ms) = forward}}                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \multicolumn{7}{c|}{\textbf{Training (ms) = forward + backward + optimization}}                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
                                                & \multicolumn{1}{l|}{}                                                         & \multicolumn{7}{c|}{Dim (Matrix dimension = Dim $\times$ Dim)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                & \multicolumn{7}{c|}{Dim (Matrix dimension = Dim $\times$ Dim)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
                                                & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Memory\\    (MB)\end{tabular}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 512}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 1024}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 2048}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 4096}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 8096}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 10240}} & \cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 20480} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 512}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 1024}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 2048}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 4096}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 8096}} & \multicolumn{1}{r|}{\cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 10240}} & \cellcolor[HTML]{8093B3}{\color[HTML]{FFFFFF} 20480} \\ \hline
Full                                            & \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F8}}                                 & \multicolumn{1}{r|}{\cellcolor[HTML]{488CC9}0.18}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{4389C8}0.13}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{478BC9}0.17}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5694CD}0.36}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{8FB9DE}1.08}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{B3CFE8}1.52}                         & \cellcolor[HTML]{FFFEFE}6.02                         & \multicolumn{1}{r|}{\cellcolor[HTML]{4288C7}0.78}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{3D85C6}0.52}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{4087C7}0.70}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5A97CE}2.02}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{B9D3EA}6.81}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}10.50}                        & \cellcolor[HTML]{FFF9F9}41.09                        \\ \hline
\multicolumn{1}{|c|}{}                          & \cellcolor[HTML]{F4F6F8}4                                                     & \multicolumn{1}{r|}{\cellcolor[HTML]{5392CC}0.32}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{609BD0}0.49}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{96BDE0}1.17}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3.18}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFBFB}11.66}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF8F8}17.57}                        & \cellcolor[HTML]{FFE0E0}69.76                        & \multicolumn{1}{r|}{\cellcolor[HTML]{468AC8}1.00}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{4E90CB}1.41}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{6CA3D4}2.93}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{CBDEEF}7.71}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFCFC}27.50}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF9F9}42.40}                        & \cellcolor[HTML]{FFDFDF}167.42                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                          & \cellcolor[HTML]{F4F6F8}32                                                    & \multicolumn{1}{r|}{\cellcolor[HTML]{5191CB}0.29}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{639CD1}0.52}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{C1D8EC}1.70}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFEFE}6.69}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF4F4}27.42}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFECEC}44.50}                        & \cellcolor[HTML]{FFAAAA}185.40                       & \multicolumn{1}{r|}{\cellcolor[HTML]{4E8FCB}1.39}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{5B98CF}2.07}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{9CC0E1}5.31}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFEFE}18.21}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF3F3}70.68}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFEAEA}114.33}                       & \cellcolor[HTML]{FFA1A1}470.72                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                          & \cellcolor[HTML]{F4F6F8}64                                                    & \multicolumn{1}{r|}{\cellcolor[HTML]{5292CC}0.32}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{6DA3D4}0.65}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.77}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFBFB}12.48}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFE8E8}52.48}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFD9D9}85.76}                        & \cellcolor[HTML]{FF5959}357.60                       & \multicolumn{1}{r|}{\cellcolor[HTML]{5C98CF}2.09}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{71A6D5}3.17}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{D8E6F3}8.36}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFBFB}31.96}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFE8E8}127.27}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFD7D7}206.83}                       & \cellcolor[HTML]{FF5656}840.00                       \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                          & \cellcolor[HTML]{F4F6F8}128                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{5493CC}0.34}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{80AFD9}0.88}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3.69}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF9F9}16.43}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFE1E1}68.55}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFCCCC}111.48}                       & \cellcolor[HTML]{FF2828}462.72                       & \multicolumn{1}{r|}{\cellcolor[HTML]{75A8D6}3.34}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{8FB8DE}4.67}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}11.02}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF9F9}40.64}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFE0E0}162.37}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFCCCC}261.56}                       & \cellcolor[HTML]{FF2727}1,069.92                     \\ \cline{2-16} 
\multicolumn{1}{|c|}{}                          & \cellcolor[HTML]{F4F6F8}256                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{4F90CB}0.27}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{81B0DA}0.90}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}4.02}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF8F8}18.46}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFDDDD}76.29}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFC7C7}124.01}                       & \cellcolor[HTML]{FF0E0E}517.53                       & \multicolumn{1}{r|}{\cellcolor[HTML]{A2C4E3}5.63}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{BFD7EC}7.11}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}14.45}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF8F8}47.79}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFDCDC}182.10}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFC6C6}292.20}                       & \cellcolor[HTML]{FF0F0F}1,188.81                     \\ \cline{2-16} 
\multicolumn{1}{|c|}{\multirow{-6}{*}{HashedNet}} & \cellcolor[HTML]{F4F6F8}512                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{4E8FCB}0.26}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{85B2DB}0.95}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}4.25}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF8F8}19.25}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFDBDB}80.00}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFC4C4}130.26}                       & \cellcolor[HTML]{FF0000}547.28                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}10.29}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}11.84}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFEFE}19.75}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF6F6}55.20}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFD9D9}197.49}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFC1C1}313.61}                       & \cellcolor[HTML]{FF0000}1,257.52                     \\ \hline
                                                & \cellcolor[HTML]{F4F6F8}4                                                     & \multicolumn{1}{r|}{\cellcolor[HTML]{5292CC}0.31}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{5594CD}0.34}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5D99CF}0.45}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{85B2DB}0.95}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.51}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3.81}                         & \cellcolor[HTML]{FFFAFA}14.83                        & \multicolumn{1}{r|}{\cellcolor[HTML]{458AC8}0.96}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{498CC9}1.16}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{4C8ECA}1.30}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{6AA1D3}2.82}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{C0D7EC}7.16}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}10.84}                        & \cellcolor[HTML]{FFF9F9}41.06                        \\ \cline{2-16} 
                                                & \cellcolor[HTML]{F4F6F8}32                                                    & \multicolumn{1}{r|}{\cellcolor[HTML]{5594CD}0.34}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{5594CD}0.35}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{629CD1}0.51}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{87B3DB}0.97}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.55}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3.98}                         & \cellcolor[HTML]{FFFAFA}14.90                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5091CB}1.51}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{5292CC}1.59}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5996CE}1.94}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{74A7D6}3.30}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{CEE0F0}7.87}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}12.11}                        & \cellcolor[HTML]{FFF9F9}43.50                        \\ \cline{2-16} 
                                                & \cellcolor[HTML]{F4F6F8}64                                                    & \multicolumn{1}{r|}{\cellcolor[HTML]{5192CC}0.30}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{5494CD}0.34}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5A97CE}0.41}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{82B0DA}0.91}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.59}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3.95}                         & \cellcolor[HTML]{FFF9F9}15.42                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5C98CF}2.08}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{5D99CF}2.15}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{619BD0}2.36}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{7CADD8}3.73}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{DDEAF5}8.63}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}12.71}                        & \cellcolor[HTML]{FFF8F8}45.18                        \\ \cline{2-16} 
                                                & \cellcolor[HTML]{F4F6F8}128                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{4E8FCB}0.26}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{4F90CB}0.27}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5896CE}0.39}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{7DADD9}0.85}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.54}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.66}                         & \cellcolor[HTML]{FFFAFA}15.03                        & \multicolumn{1}{r|}{\cellcolor[HTML]{71A6D5}3.16}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{70A5D5}3.12}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{78AAD7}3.52}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{91B9DE}4.76}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{F7FAFC}9.93}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}14.47}                        & \cellcolor[HTML]{FFF7F7}49.73                        \\ \cline{2-16} 
                                                & \cellcolor[HTML]{F4F6F8}256                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{478BC9}0.17}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{488CC9}0.18}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{5091CB}0.29}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{77A9D7}0.77}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.47}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.56}                         & \cellcolor[HTML]{FFFBFB}11.12                        & \multicolumn{1}{r|}{\cellcolor[HTML]{9CC0E1}5.32}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{9CC1E2}5.35}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{A4C6E4}5.73}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{BDD5EB}7.00}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}12.22}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFEFE}16.73}                        & \cellcolor[HTML]{FFF6F6}56.08                        \\ \cline{2-16} 
\multirow{-6}{*}{ROAST}                         & \cellcolor[HTML]{F4F6F8}512                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{3D85C6}0.04}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{4087C6}0.08}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{4A8DCA}0.21}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{73A7D5}0.72}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FCFDFE}2.44}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2.55}                         & \cellcolor[HTML]{FFFCFC}9.95                         & \multicolumn{1}{r|}{\cellcolor[HTML]{F5F9FC}9.82}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{F7FAFC}9.91}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}10.33}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}11.63}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFEFE}16.96}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFDFD}21.56}                        & \cellcolor[HTML]{FFF6F6}55.60                        \\ \hline
\end{tabular}}

\end{table}

==> tables/nlp_t1.tex <==
\begin{table}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|ll|ll|ll|ll|}
\hline
Datasets                  & Train data points & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Original \\  (108M)\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Rz 10x \\ (10.9M)\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Rz 100x\\  (1.2M)\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Rz 1000x\\    (232K)\end{tabular}} \\ \hline
                          &                   & \multicolumn{1}{l|}{loss}                         & acc                          & \multicolumn{1}{l|}{loss}                        & acc                         & \multicolumn{1}{l|}{loss}                        & acc                         & \multicolumn{1}{l|}{loss}                          & acc                          \\ \hline
tweet-eval ( hate-speech) & 9K                & \multicolumn{1}{l|}{0.568}                        & 0.708                        & \multicolumn{1}{l|}{0.544}                       & 0.722                       & \multicolumn{1}{l|}{0.576}                       & 0.702                       & \multicolumn{1}{l|}{0.578}                         & 0.720                        \\ \hline
tweet-eval ( sentiment)   & 45K               & \multicolumn{1}{l|}{0.755}                        & 0.671                        & \multicolumn{1}{l|}{0.758}                       & 0.655                       & \multicolumn{1}{l|}{0.762}                       & 0.670                       & \multicolumn{1}{l|}{0.824*}                        & 0.619*                       \\ \hline
ag-news ( news )          & 120K              & \multicolumn{1}{l|}{}                             &                              & \multicolumn{1}{l|}{}                            &                             & \multicolumn{1}{l|}{}                            &                             & \multicolumn{1}{l|}{}                              &                              \\ \hline
yelp-polarity ( review)   & 560K              & \multicolumn{1}{l|}{}                             &                              & \multicolumn{1}{l|}{}                            &                             & \multicolumn{1}{l|}{}                            &                             & \multicolumn{1}{l|}{}                              &                              \\ \hline
amazon-polarity (review)  & 3.6M              & \multicolumn{1}{l|}{}                             &                              & \multicolumn{1}{l|}{}                            &                             & \multicolumn{1}{l|}{}                            &                             & \multicolumn{1}{l|}{}                              &                              \\ \hline
\end{tabular}}
\caption{Model = BERT-BASE (100M paraemeters) , Different sized datasets. Evaluated every 100 iterations. Max 10 epochs.}
\label{tab:my-table}
\end{table}

==> tables/vision_datasets.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|}
\hline
\textbf{Datasets} & \textbf{train size} & \textbf{test size} \\ \hline
cifar-10          & 50K                 & 10K                \\ \hline
cifar-100         & 50K                 & 10K                \\ \hline
food-101          & 75.7K               & 25.2K              \\ \hline
\end{tabular}
\caption{Datasets used for text-classification task. All datasets are taken from HuggingFace and use the standard test/train split provided by them}
\label{tab:nlpds}
\end{table}

==> text/abstract.tex <==
%In many domains, deep learning models are becoming more accurate. However, this boost in accuracy comes at a disproportionate increase in model sizes. Large models are challenging to train, requiring advanced computational capabilities, not to mention the exorbitant costs incurred during training and hyper-parameter tuning. Additionally, large models are expensive for real-world deployment; the sheer size of large models makes them impossible to deploy on edge and mobile devices. To solve this problem, inference is usually performed on cloud servers, but this can cause long delays and compromise data privacy.
%Thus, 
The deployment cost and latency of deep learning is dramatically affected by the model size.  Models like BERT cannot be deployed on edge devices and mobiles due to its sheer size. As a result, most advances in Deep Learning are yet to reach the edge. Model compression has sought much-deserved attention in literature across domains of NLP, vision, and recommendation. This paper proposes a model-agnostic, cache-friendly model compression approach: Random Operator Access Specific Tile (\roach) hashing. 
{\roach} collapses the parameters by clubbing then through a lightweight mapping. Notably, while clubbing these parameters, {\roast} smartly utilizes cache hierarchies by aligning the memory access pattern with the parameter access pattern. 
%tunes the mapping to align with pattern in which the parameters are accessed in the algorithmic implementation of the operation being performed.
{\roach} is up to ${\sim}25\times$ faster to train and ${\sim}50\times$ faster to infer than popular parameter sharing method HashedNet. Additionally, {\roast} introduces global weight sharing, which is empirically and theoretically superior to local weight sharing in HashedNet and can be of independent interest in itself.  With {\roach}, we present the first compressed BERT which is 100$\times$-1000$\times$ smaller but does not result in quality degradation. These compression levels on universal architecture like transformers are promising for the future of SOTA model deployment on resource-constrained devices like mobile and edge devices. We hope our work gets adopted in practice. 

==> text/introduction.tex <==
% Model are becoming larger 
Models across different domains, including Natural Language Processing (NLP), Computer Vision (CV), and Information Retrieval (IR), are exploding in size.
State-of-the-art (SOTA) results in these domains are being obtained at a disproportionate increase in model sizes, questioning the sustainability of deep learning~\cite{thompson2021deep}.
For instance, SOTA architectures for vision include VGG~\cite{vgg} (~150M params, 0.6GB) and ViT~\cite{vit} (upto 304M params, 1.2GB). Additionally, SOTA NLP architectures include BERT~\cite{devlin2018bert} (340M params, 1.36GB), GPT-2~\cite{gpt} (1.5B params, 6GB), MegatronLM~\cite{megatron} (8.3B params, 34GB), T5~\cite{t5} (11B params, 44GB), T-NLG~\cite{nlg} (17B params, 68GB), GShard~\cite{gshard} (600B params, 2.4TB) and so on.
Similarly, industrial-scale recommendation models such as DLRM~\cite{DLRM19} can have up to 100 billion parameters.
Models as large as these can cause many issues in various aspects.

%\textbf{Deployment of models}
Many real-world applications require deploying models on edge and mobile devices; however, SOTA models cannot be deployed due to their large sheer size.
In general, such models are deployed on high-end servers, and applications on devices need to communicate data to these servers to retrieve the results.
This mechanism not only makes the service slow due to communication between devices and servers but also creates a data privacy concern as private data are sent to remote servers. 

%\textbf{Training and inference with large models}
%Training large SOTA models requires elaborate computational resources and costly power consumption.
%For instance, it is estimated that training the BERT model, along with hyperparameter tuning, requires around 200K USD~\cite{sharir2020cost}.
%Indeed, such a training process is beyond the scope of an average industrial company, let alone academic institutions.
Additionally, for any distributed training and particularly federated learning~\cite{} model size is the primary bottleneck in communication. The communication footprint is directly proportional to model size. 
%Furthermore, skillfully engineered systems, that are beyond the capabilities of a general machine learning user, are needed for making training such large models feasible.
%Similar to training, inference of these models on a distributed system is slow due to involved communication costs.

%\textbf{Model compression}
Compressing large models to small sizes come with immediate benefits.
For example, Diamos et al.~\cite{diamos2016persistent} showed that if a single RNN layer can fit in registers, then it leads to $146\times$ faster inference.
Also, Desai et al.~\cite{robez} showed that by compressing the DLRM model $1000\times$ and using a single GPU instead of 8 GPUs, we could get $3\times$ faster inference at a lower cost.
A smaller memory footprint directly affects all aspects of model training and inference.
Specifically, storing a model on a single GPU instead of multiple GPUs can lead to faster training and inference, lower costs, and easier deployment with the possibility of deploying on edge and mobile devices.
Also, compressed models can eliminate the need for solving engineering challenges that come with large models.

% model compression in literature
There has been ample evidence in the literature that models often can be compressed to a large extent.
For instance, Denil et al.~\cite{denil2013predicting} showed that we could predict all parameters of a model using only 5\% of the parameters.
Since then, there has emerged research in model compression across various domains.
A variety of model compression paradigms now exist in literature like pruning~\cite{Han2016DeepCC}, quantisation~\cite{Han2016DeepCC}, knowledge distillation~\cite{modelcompression}, parameter sharing~\cite{hashtrick,robez}, and low rank decomposition~\cite{hrinchuk2020tensorized, ttrec}.
We will discuss each of these paradigms in section \ref{sec:related}. This paper follows the parameter-sharing world of model compression.
Also, we will focus on the NLP compression for the sake of discussion in this paper.
However, it should be noted that our proposed model compression technique is model agnostic and can be applied to any model in any domain.

% parameter sharing in NLP.
%\textbf{Parameter sharing and {\roast}}

{\bf \color{red} Anshu: Too much fixated on hashed net! We can even remove almost all of this. Well, think about this, the best compression the world has seen on BERT is 18x, you are giving them 100x+. Now hashednet is just one of the many ideas out there for a while and did not achieve good results. You dont have to justify more than that here.}

In HashedNet~\cite{hashtrick}, authors presented a way to compress matrices in MLP models by randomly mapping weights in the matrix into a small parameter repository.
Surprisingly, HashedNet, in its original form, was never evaluated on large NLP models like BERT.
We evaluated HashedNet with different memory sizes and found that its latency is high because of the random access pattern, as shown in section~\ref{sec:triton}.
Parameter sharing approaches like character-aware language~\cite{kim2016character} models and slim embeddings~\cite{li2018slim} are applied only to embedding compression in NLP.
However, embedding tables are no longer the only memory-consuming computational module of NLP models.
For instance, BERT-base (108M) parameters have around 80\% parameters in attention blocks and other MLP layers and only 20\% parameters in embedding tables.
We propose {\roachfull} (\roach) hashing, a parameter sharing approach, which can be applied to all computational modules of 
a model such as MLP layers, attention blocks, convolution layers, and embedding tables.
{\roast} leverages a recent result in hashing, which shows that chunk-based hashing is theoretically superior to usual feature hashing~\cite{robez}.
{\roach} proposes a tile-based hashing scheme that is tuned to the memory access pattern of the algorithmic implementation of the operation being performed. This resolves the latency issues of HashedNet by coalescing memory accesses. 
Thus, {\roast} gives us an efficient knob on the memory footprint of the model without affecting its functional form.
Additionally, {\roach} also proposes global weight-sharing as opposed to local weight-sharing presented in HashedNet.
As we shall see, global weight-sharing is both empirically and theoretically superior to local weight sharing and might be of independent interest to the community.  

% review of results.
We evaluated {\roach} compression on the Transformer-like model. Transformers are emerging as a universal architecture showing good results in all the three domains, NLP~\cite{devlin2018bert,vaswani2017attention}, CV~\cite{vit} and IR~\cite{moreira2021transformers}.
With {\roach}, we could compress the BERT model as much as $100\times-1000\times$ without any loss of quality in training-from-scratch on text-classification task. 
While our experiments cannot be compared in an apples-to-apples fashion to other compression results in the literature, none of the existing compression techniques have shown compression as large as $100\times$ without loss of quality.
A $100\times$ {\roach}ed BERT model is small enough to fit the cache of CPUs and is easily deployable on mobile/edge devices. 

\textbf{Limitations of {\roach}:} One of the goals of model compression, apart from reducing memory usage, is to reduce computational workload for deployment. {\roach}, however, our current implementation is not optimized enough to decrease computation; it only decreases the memory footprint of a model. Reducing computation with a small memory is left for future work. However, it should be noted that reducing the memory footprint itself can reduce computation latency and power consumption significantly.
As shown in \cite{han2016eie}, accessing memory from RAM is 6400$\times$ costlier than 32bit INT ADD and 128$\times$ costlier than on-chip SRAM access in terms of energy consumption. Additionally, RAM access generally is ${\sim}100 \times$ slower than a floating-point operation. This shows that reducing memory footprint so that model can fit in faster memory can, at times, be much more impactful than reducing the computational burden.


% 2. Smaller models necessary for deployment. (all arguments from NLP survey)
% 3. Easier to train; faster to infer
% 4. short background.
% 5. short introduction to our method ROACH.
% 6. A small paragraph on contributions.
% 7. caveats

==> text/robez.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.25]{fig/model_compression_bert_1.png}
    \caption{Generic model compression with operator specific blocking for BERT as an example.}
    \label{fig:mc}
\end{figure}

% Fundamental idea
Random Operator Access Specific Tile ({\roast}) hashing proposes an efficient model-agnostic parameter sharing-based model compression approach. {\roast} disentangles the functional form and memory footprint used by the model, providing a separate knob for controlling memory usage. In contrast to the Local memory sharing(LMS) performed in HashedNet, in {\roast} we perform Global Memory Sharing (GMS), where all model parameters across the different computational modules share a single memory array. GMS  performs much better than LMS, both in theory and practice. Additionally,  {\roast} proposes operation(or algorithm)-specific tile hashing instead of hashing every element, coalescing the memory specific to access pattern and improving cache-line efficiency. As we shall see, {\roast} can be up to 50$\times$ faster than HashedNets, demonstrating the effect of memory-coalescing. In the next section, we discuss the basic operations of deep learning, which interact with weight memory, and how {\roast} hashing is used in each case.

% Deep learning models. 
\ssubsection{Operations in Deep learning interacting with weight memory with \roach }
Any model can be seen as a sequence of operations $\{\mathcal{O}_i(A_i, W_i)\}_{i=1}^n$ where $W_i$ is the weight used in operation $\mathcal{O}_i$; $A_i$ are the inputs to this operation and generally includes the input data and outputs of previous operations. Depending on the granularity, some operations may not interact with the weights. In deep learning models, the operations interacting with weight-memory can mostly, if not completely,be composed of two basic operations (1) matrix multiplication and (2) memory lookup. And hence in {\roach} we discuss operation-specific tiling for these operations. (Note that matrix multiplication with weight matrix can be seen as lookup the entire matrix followed by matrix multiplication. However, this will mean we have to recover entire matrix in memory which would defeat the purpose of weight-sharing to reduce memory footprint.) The \todo{table} \ref{tab:paramtable} shows the contribution of different operations to memory parameters in various models. Let us look at these two operations and hashing schemes proposed by {\roach} for them. We should emphasize that while we only discuss two operations here, the philosophy of {\roach} can be extended to any operation to give an efficient kernel implementation.
%However, the hashing of subset of weights corresponding to a particular operation uses a different blocking scheme which can be tuned w.r.t how the memory is accessed during operations. The purpose behind this choice is to improve coalesced access of weights and reduce number of memory fetches. As shown in the figure \ref{fig:mc}, we use block shapes of 1D array for embeddings whereas block shapes of 2D arrays for matrix multiplication.
% basic operations in models
%The model architecture can have components such as embedding tables, feed-forward networks, attention blocks , convolutions and so on. It is interesting to note that all of these operations can be decomposed into two fundamental operations

\textbf{Memory look-up:} In the context of deep learning models, memory look-up is an operation that is largely associated with embedding tables. However, we can also implement relatively small-sized model components, such as bias vectors, etc., via look-ups. ( for example, we recover the bias vector into memory and then use it)  \textbf{1D tile hashing in memory-lookup:}
In order to make the hashing scheme system-friendly, we note that the access in a vector is sequential. Hence the vector is divided into chunks of a particular size. Now each of these chunks is located randomly in the {\roach} array using GPU friendly universal hashing \cite{univ-hash}. The coalesced access causes the number of cache-line fetches to be similar in number to when we retrieve the vector in original setting. 
%The hashing scheme  is illustrated in figure \ref{fig:mc}. ROBE-Z \cite{robez} introduced this hashing scheme for embedding tables. We generalize their kernel to implement our lookup operation. 
%Recall that in {\roach}, these computational blocks share memory with each other as well as matrix multiplication blocks.

\textbf{Matrix-multiplication:} Matrix multiplication  (MM) is another essential fundamental operation performed on weights of model. For instance, MM followed by the non-linear activation is the only elementary operation in feed-forward networks. Also, convolutions are MM  of input patches with weight matrix. Furthermore, the attention block in transformers also contains MM of inputs with three matrices (K, Q  and V) which are then used to compute attention scores. \textbf{2D tile-hashing in matrix multiplication:}
The matrix multiplication cannot follow the same 1-D tiling scheme used for the look-up operation. In order to decide the tiling for MM, we look at the implementation of MM. On GPUs, MM is implemented as a 2D-tiled block-multiplication algorithm to optimize the shared-memory usage. Specifically, the two matrices involved in multiplication, say $A\in R^{M \times K}$ and $B \in R^{K \times N}$ are divided into tiles of size $m \times k$ and $k \times n$ respectively. Then $g$ tiles are grouped to form a super 2-D tile. $m,k,n$ and $g$ are parameters of this algorithm tuned to get the best performance. Multiplication implementation then proceeds by bringing super tiles from matrices A and B into shared memory. These super tiles are multiplied and the result is updated. This algorithm also aligns well with new tensor cores on NVIDIA GPU
%, which provide $4\times4$ matrix multiplication hardware. 
In {\roach}, we propose to coalesce the super tile into the memory. We hash the super tile, identified by its coordinates in the matrix, into the memory and store it in a row-major format. This is illustrated in figure \ref{fig:mc}. As discussed in section \ref{sec:triton}, we implement our forward and backward kernel for MM (\roach-MM) in triton \cite{triton}. As we shall see \roast-MM is orders of magnitude faster than HashedNet kernel (also implemented in triton)

\ssubsection{Global memory sharing.}
\textbf{Initialization adjustment}
HashedNet proposed "local memory sharing"(LMS), which states that each layer will have independent compressed memory.
In contrast  {\roach} proposes "global memory sharing" (GMS), wherein we share memory across the computational modules. However, computational modules cannot directly use the parameters stored in the {\roast} array as each module weight requires initialization and optimization at different scales. For instance, in Xavier's initialization \cite{glorot2010understanding}, weights of a node are initialized with distribution $U(-1/\sqrt{n}, 1/\sqrt{n})$ where n is the number of inputs to the node. In GMS, we must ensure that each computational module gets weights at the required scale. In order to achieve this, we first initialize the entire {\roach} parameter array with values from the distribution $U(-1/C,1/C)$ for some constant C.  
Then for each computational module, we scale the weights retrieved from the {\roach} array by a factor of $C/\sqrt{n}$ where n is the number of inputs to the nodes in this module.

\textbf{Global memory sharing enables better functional expressivity}
A simple argument in favor of GMS compared to LMS stems from number of possible functions that can be represented using fixed parameter memory. Consider we have a parameter memory of size $m$ with distinct parameter values and $k$ modules with total weight sizes of $n_1,n_2, ... n_k$. Let total weight size be $n=n_1+n_2+...+n_k$. In global memory sharing, number of functions we can form with this fixed memory is $m^n$. However, in local memory sharing where each module gets its own private memory of parameters say of sizes $m_1, m_2, m_3, .. m_k$ where $m = m_1+m_2+..m_k$, the number of possible functions is $m_1^{n_1} m_2^{n_2} ... m_k^{n_k}$ which is strictly less than $m^n$ and can be orders of magnitude smaller depending on exact values of $m_i$ and $n_i$. We show in section \ref{sec:theory} that GMS is better than LMS in terms of feature hashing quality and provide empirical evidence of its superiority in section \ref{sec:robez_exp}

\ssubsection{ Forward and Backward Passes}
\textbf{Forward pass:} Recall that the forward pass of the model is a series of operations $\{\mathcal{O}_i(A_i, W_i)\}$. Each operation that interacts with the weight memory via $W_i$ can be composed of two operations; either memory look-ups or matrix multiplication. Conceptually, the operation in {\roach} is equivalent to recovering the weight $W_i$ from the {\roach} array, and then performing the exact operation $\mathcal{O}_i$. For lookup operation, let the 1D tile be of size Z. Similarly let the 2D tile be of size $Z_1 \times Z_2$ for MM operation. Then recovered weight can be written as
\begin{align*}
    &W_{lu}[i] = \lambda(W_{lu}) *  \mathcal{M}[h(C(i, Z)) + O(i, Z)]  \\
    &\quad W_{mm}[i,j] = \lambda(W_{mm}) * \mathcal{M}[h(C(i, Z_1), C(j, Z_2)) + O(i,j, Z_1,Z_2)] \\
    &C(i, Z)) = i // Z  \quad \quad O(i,Z) = i \% Z \quad \quad O(i,j,Z_1,Z_2) = Z_2*(i\%Z_1) + j \% Z_2
\end{align*}
Where $W_{lu}$ and $W_{mm}$ are recovered vector for lookup and matrix for MM operation respectively. Also, $C(i, Z)$ computes the tile number to which $i$ belongs to in  lookup vector blocking.$O(i, Z)$ computes the offset within the 1D tile and $O(i,j, Z_1,Z_2)$ is the row-major offset in 2D tile. Also $\lambda$ returns the scale we want to use for that particular module. We use universal hashing function $h: \mathbf{N}^k \rightarrow \{0,...,m'-1\}$. $k$ depends on how many integers we use to identify a particular tile. The universal hash function can be defined as 
\begin{equation}
    h(x_1, ... , x_k) = (A_0 + A_1 x_1 + A_2 x_2 + .. + A_k x_k) \% P \% m'
\end{equation}
where P is a prime number larger than $m'$ and $A_i, i \geq 1$ are integers drawn randomly from $[1,P-1]$ and $A_0$ is drawn randomly from $[0,P-1]$. For simplicity of implementation we use $m' = |\mathcal{M}| - Z$ in case of lookup and $m' = |\mathcal{M}| - Z_1Z_2$ in case of MM. It is important to note that the entire weight is never recovered completely in memory as that would defeat the purpose of model compression. Instead each memory access in the implementation of the operation just goes through the hash function in {\roach}. 

In order to implement lookup operation, we generalize the ROBE-Z kernel \cite{robez}. We implement our own kernel ROAST-MM for matrix multiplication. The forward pass for \roach-MM kernel is shown in algorithm \ref{algo:roach-mm} in appendix \ref{sec:roastmmal}

\textbf{backward pass:} The gradient of the loss w.r.t a weight in the {\roach} array is the $\lambda$-scaled aggregation of gradients of loss w.r.t all the parameters that map to this weight. For simplicity of notation consider $\theta$ as the complete parameter, $\lambda(j)$ as the scaling factor we use for the computational module that $\theta_j$ belongs to, $h$ be hashing map function.
\begin{equation}
    \nabla_{w_i} f(w) = \sum_{j , h(j) = i} \lambda(j) * \nabla_{\theta_j} f(\theta)
\end{equation}
In order to see why this works even while sharing weights across the different components of the model (like various layers of MLP , or MLP and embedding tables) , note that 
\begin{align}
    \frac{\partial f(x, g(x))}{\partial x} = \frac{\partial f(z, g(y))}{\partial z}|_{y=x, z=x} +  \frac{\partial f(z, g(y))}{\partial y} |_{y=x, z=x}
\end{align}
This essentially states that we can rename the parameters from different computational modules which are mapped to single weight, and compute gradients w.r.t renamed variables. The gradient w.r.t to the weight then is just sum of the individual gradients. Proof of this is presented in appendix \ref{sec:gradexp}.

